Optimal Vehicle Dispatching Schemes via Dynamic Pricing

Over the past few years, ride-sharing has emerged as an effective way to relieve traffic congestion. A key problem for these platforms is to come up with a revenue-optimal (or GMV-optimal) pricing scheme and an induced vehicle dispatching policy that incorporate geographic and temporal information. In this paper, we aim to tackle this problem via an economic approach. Modeled naively, the underlying optimization problem may be non-convex and thus hard to compute. To this end, we use a so-called "ironing" technique to convert the problem into an equivalent convex optimization one via a clean Markov decision process (MDP) formulation, where the states are the driver distributions and the decision variables are the prices for each pair of locations. Our main finding is an efficient algorithm that computes the exact revenue-optimal (or GMV-optimal) randomized pricing schemes. We characterize the optimal solution of the MDP by a primal-dual analysis of a corresponding convex program. We also conduct empirical evaluations of our solution through real data of a major ride-sharing platform and show its advantages over fixed pricing schemes as well as several prevalent surge-based pricing schemes.

==> conclusion.tex <==
\section{Conclusions and Future Work}\label{sec:conclusion}
In this paper, we propse a novel general model for ride-sharing platform to find revenue-optimal(or welfare-optimal) pricing scheme. With such a model, we convexify this optimization problem by "ironing" techinique and formalize it to a Markov decision process. An efficient algorithm is given to attain revenue-optimal randomized pricing scheme. We also characterize the optimal solutions from an economic perspective and give some insights for real applications. In our experiment, we compare our algorithm with two pricing schemes under static and dynamic environments respectively. Our solutions outperform the benchmark policies both on revenues and the ability of balacing demand and supply.

We believed that our model can be used for real applications. In the future, we plan to further investigate on the dual problem, which has more economic interpretation and pratical significance. [cmj: more future work]

==> dynamic.tex <==
\section{Generalization for Dynamic Environment}\label{sec:dynamic}
In this setting, we consider a more general case where the objective function
$\hat{g}_\tau(q|e)$ is time-dependent. The information about supply and demand
curves can not be predicted accurately for infinite terms in reality, thus we
consider dynamic environment with finite horizon, which is more consistent with
the real situation. 

Given the convex program for static environment with infinite horizon, the
convex program for the dynamic environment with finite horizon is rather
straightforward, i.e.,
\begin{equation}
\tag{P.2} \label{prog:dynamic}
\begin{aligned}
	\max \quad &  \sum_{\tau = 1}^{T} \sum_{e\in E}\hat{g}_\tau(q|e)  \\
	\text{s.t.} \quad
		&  \sum_{v\in V}w_\tau (v) = 1,~ \forall \tau  \\
		&  \sum_{\vout(v)}q_\tau(e) \leq w_\tau (v),~ \forall v , \tau\\
		&  w_{\tau+1}(v) - w_\tau(v)= \sum_{\vin(v)}q_\tau(e)+\sum_{\vout(v)}q_\tau(e) ,~ \forall v, \tau \\
		& w_\tau(v)\ge 0, q_\tau(e) \ge 0,~\forall v, \tau
\end{aligned}
\end{equation}

% \begin{gather*}
% \max \lim\limits_{\tau \rightarrow \infty}\sum_{\tau = 1}^{T}\gamma_{e,\tau}
% \end{gather*}
% such that
% \begin{eqnarray*}
% 	\sum_{v\in V}w_\tau (v) &=&1\quad \forall \tau \in T\\
% 	\sum_{t\in V, e=(v,t)\in E}q_\tau(e) &\leq& w_\tau (v) \quad \forall v \in V ,\; \forall \tau \in T\\
% 	w_\tau(v)-\sum_{t\in V, e=(v,t)\in E}q_\tau(e)+\sum_{s\in V, e=(s,v)\in E}q_\tau(e) &=&w_{\tau+1}(v)\quad \forall v \in V,\; \forall \tau \in T \\
% 	\gamma_{e,\tau} -g_\tau(q|e) &\leq & 0 \quad \forall e \in E,\; \forall \tau \in T
% \end{eqnarray*}


==> general.tex <==
\section{Generalizations}\label{sec:general}

Despite of the simple structure of our model, it is flexible
enough to extend to many practically important generalizations.

\paragraph{Non-uniform distances}


\paragraph{Dynamic driver population}
Similar to the uniform distance assumption, in our framework, we
can safely remove the constraint on the fixed driver population.
Instead, we can apply different constraints on the driver
population in different periods, or one single constraint that
specifies the total driver population accumulated overtime. In
particular, we find the following special cases quite interesting:
\begin{itemize}
  \item {\bf Fixed total driver population accumulated overtime}.
        To do this, one can simply replace the driver population
        constraints on each period to one single constraint on the
        total accumulated driver population. In fact, such a
        constraint can be interpreted as that there is a fixed
        driver work hour supply. According to \cite{chen2015dynamic}, it is a very
        realistic assumption given that most drivers have
        their fixed target working time per week.
  \item {\bf Unlimited driver supply, but with increasing marginal
        cost}. In stead of placing a hard constraint on the driver
        supply, it is more realistic to allow the platform to have
        unlimited power of attracting more drivers but at
        increasing marginal cost. To incorporate this with our
        convex program, one can simply remove the hard driver
        population constraints and subtract the additional marginal
        cost of attracting more drivers from the objective. As long
        as the marginal cost is weakly increasing, the new program
        is still convex.
\end{itemize}

% \paragraph{Non-uniform requests}
% In our model, we normalize requests on each edge to be 1. 

